An Ensemble Approach Towards Adversarial Robustness

It is a known phenomenon that adversarial robustness comes at a cost to natural accuracy. To improve this trade-off, this paper proposes an ensemble approach that divides a complex robust-classification task into simpler subtasks. Specifically, fractal divide derives multiple training sets from the training data, and fractal aggregation combines inference outputs from multiple classifiers that are trained on those sets. The resulting ensemble classifiers have a unique property that ensures robustness for an input if certain don't-care conditions are met. The new techniques are evaluated on MNIST and Fashion-MNIST, with no adversarial training. The MNIST classifier has 99% natural accuracy, 70% measured robustness and 36.9% provable robustness, within L2 distance of 2. The Fashion-MNIST classifier has 90% natural accuracy, 54.5% measured robustness and 28.2% provable robustness, within L2 distance of 1.5. Both results are new state of the art, and we also present new state-of-the-art binary results on challenging label-pairs.

==> liter.tex <==

\section{Related Work} \label{sec:liter}

There are a variety of approaches to robustness \cite{meng2017magnet,towards}.
Adversarial training with an $L_{\infty}$ adversary is perhaps the most popular one.
Indeed, it results in excellent $L_{\infty}$ robustness on MNIST \cite{mit}, although the effect on CIFAR is less satisfactory; \cite{mindistort} showed that, for a small network, it increases the provable $L_{\infty}$ robustness; \cite{l2nnn} reported that it also helps improving $L_2$ robustness.
It is both a data augmentation scheme and a method to flatten gradients around training data points.
From the latter perspective, gradient regularization \cite{ross2018improving} is strongly related and an alternative.
Other works aim to bound a network's responses to input perturbations over the entire input space, and \cite{kolter,raghu,wong2018scaling} achieved provable guarantees on $L_{\infty}$ robustness.

$L_2$ robustness is less understood and perhaps more difficult.
Adversarial training with an $L_2$ adversary has been reported in \cite{tradeoff} and the performance is not satisfactory.
Prior to this paper, \cite{l2nnn,towards,nbr} are the only works that have shown substantial $L_2$ robustness, and Section~\ref{sec:results} includes all of them in the comparisons.
\cite{l2nnn} has provable guarantees on $L_2$ robustness.

The robustness-accuracy trade-off has been reported in most of the prior works.
It remains an open question whether some loss of nominal accuracy is an inevitable cost of robustness.
\cite{nbr} achieved a more favorable trade-off using divide-and-conquer and reasoning.
This paper shares the same strategy and improves it significantly with the two new techniques.


